Best Axes Composition Extended: Multiple Gyroscopes and Accelerometers Data Fusion to Reduce Systematic Error

Multiple rigidly attached Inertial Measurement Unit (IMU) sensors provide a richer flow of data compared to a single IMU. State-of-the-art methods follow a probabilistic model of IMU measurements based on the random nature of errors combined under a Bayesian framework. However, affordable low-grade IMUs, in addition, suffer from systematic errors due to their imperfections not covered by their corresponding probabilistic model. In this paper, we propose a method, the Best Axes Composition (BAC) of combining Multiple IMU (MIMU) sensors data for accurate 3D-pose estimation that takes into account both random and systematic errors by dynamically choosing the best IMU axes from the set of all available axes. We evaluate our approach on our MIMU visual-inertial sensor and compare the performance of the method with a purely probabilistic state-of-the-art approach of MIMU data fusion. We show that BAC outperforms the latter and achieves up to 20% accuracy improvement for both orientation and position estimation in open loop, but needs proper treatment to keep the obtained gain.

==> archive/00b_notes.tex <==
check referencing to equations

V is M

==> archive/_03b_acc_background.tex <==
\color[rgb]{0.00,0.35,0.00}
\section*{\mf{Acc}}

\noindent\mf{\\$a$ - acc in local frame\\$\alpha$ - acc in world frame}

Measurements of high-end factory-calibrated MEMS gyroscopes can be modeled as~in \cite{nikolic2016characterisation}:
\begin{align}
    \lf{I}\tilde{\vect{a}}(t) &= \lf{I}\vect{a}(t) + \vect{b}_a(t) + \vect{\eta}_a(t),
    \label{eq_perf_acc_cont}
\end{align}
where $\lf{I}\tilde{\vect{\omega}}(t)$ is the measured value by the sensor,  $\lf{I}\vect{\omega}(t)$ the true angular velocity and $\vect{\eta}_g(t)$ is a Wiener process.
The term $\vect{b}(t)$ is the slow varying continuous-time bias modeled as
\begin{align}
    \dot{\vect{b}_a}(t) = - \frac{1}{\tau_{b_a}} \vect{b}_a(t) + \vect{\epsilon}_a(t),
    \label{eq_ct_bias_acc}
\end{align}
where $\vect{\epsilon}(t)$ is a Wiener process and
$\tau_b$ is a correlation time of bias~\cite{crassidis2006sigma}.

%\mf{Exp is not defined above, below only}
%\mf{$\Exp(\lf{I_g}\theta_{I_a}) = \lfR{i_g}\rf{I_a}$}
\begin{align}
    \lf{I}\vect{a}(t) &= \lfR{I_g}\rf{I_a}\,[C_a\,\lf{I}\tilde{\vect{a}}(t) - \vect{b}_a(t) - \vect{\eta}_a(t)].
\label{eq_cor_acc_cont}
\end{align}

The discrete-time model of (\ref{eq_cor_acc_cont})  accordingly is
\begin{align}
    \lf{I}\vect{a}(t_k) &= \lfR{I_g}\rf{I_a}\,[C_a\, \lf{I}\tilde{\vect{a}}(t_k) - \vect{b}_a(t_k) - \vect{n}_a(t_k)],
    \label{eq_cor_acc_dis}
\end{align}
where the continuous-time bias is now  expressed by the discrete-time equation
\begin{align}
    \Delta \vect{b}_a(t_k) = - \gamma_a \vect{b}_a(t_k) + \vect{n}_{b_a}(t_k)
    \label{eq_bias_dis_acc}
\end{align}
and $\Delta \vect{b}(t_k)$ is the difference of bias
\begin{equation}
    \Delta \vect{b}_a(t_k) \triangleq \vect{b}_a(t_{k+1}) - \vect{b}_a(t_k).
\end{equation}

The parameter $\gamma$ is a dimensionless coefficient that takes into account bias correlation time as described in the appendix of~\cite{crassidis2006sigma}. The random variable $\vect{n}_{b_a} \sim \mathcal{N}(\vect{0}, \Sigma_{\vect{n}_{b_a}})$ and $\vect{n}_a \sim \mathcal{N}(\vect{0}, \Sigma_{\vect{n}_a})$.

\mf{New}
%\begin{align}
\begin{equation}
    \lf{I}\vect{\alpha}(t) = \lfR{W}\rf{I}(t)\, \lfR{I_g}\rf{I_a}\,[C_a\,\lf{I}\tilde{\vect{a}}(t) - \vect{b}_a(t) - \vect{\eta}_a(t)] - \vect{g}.
\label{eq_cor_acc_cont2}
\end{equation}
%\end{align}

The discrete-time model of (\ref{eq_cor_acc_cont2})  accordingly is
%\begin{align}
\begin{equation}
    \lf{I}\vect{\alpha}(t_k) = \lfR{W}\rf{I}(t_k)\, \lfR{I_g}\rf{I_a}\,[C_a\, \lf{I}\tilde{\vect{a}}(t_k) - \vect{b}_a(t_k) - \vect{n}_a(t_k)] - \vect{g},
    \label{eq_cor_acc_dis2}
\end{equation}    
%\end{align}

\subsection{Kinematic Model}\label{sec_kinem_acc}

Accordingly, the integration of the linear acceleration $\lf{I}\vect{a}({t_k})$ at the IMU frame is exactly calculated by
\begin{align}
    \lf{W}\vect{v}\rf{I}({t_{k+1}}) &= \lf{W}\vect{v}\rf{I}(t_{k}) + \lf{I}\vect{\alpha}(t_k) \Delta t_k,\\
    \lf{W}\vect{p}\rf{I}({t_{k+1}}) &= \lf{W}\vect{p}\rf{I}(t_{k}) + \lf{W}\vect{v}\rf{I}(t_{k}) \Delta t_k + \frac{1}{2}\lf{I}\vect{\alpha}(t_k) \Delta t_k^2,
\end{align}



The orientation of the Master frame $\{M\}$, given any of the $i$-th IMUs can be computed by the similar equation:
%\mf{v?}
%\begin{align}
%    \lf{W}\vect{p}\rf{M}({t_{k+1}}) &= \lfR{W}\rf{I}(t_k+1) \lf{I}\vect{p}\rf{M} + \lf{W}\vect{p}\rf{I}(t_{k+1}),
%\end{align}

\begin{align}
    \lf{M}\vect{\alpha}(t_{k+1}) &= \lfR{W}\rf{M}(t_k) \lf{M}\vect{a}(t_k),\\
    \lf{W}\vect{v}\rf{M}({t_{k+1}}) &= \lf{W}\vect{v}\rf{M}(t_{k}) + \lf{M}\vect{\alpha}(t_k) \Delta t_k,\\
    \lf{W}\vect{p}\rf{M}({t_{k+1}}) &= \lf{W}\vect{p}\rf{M}(t_{k}) + \lf{W}\vect{v}\rf{M}(t_{k}) \Delta t_k + \frac{1}{2}\lf{M}\vect{\alpha}(t_k) \Delta t_k^2,
\end{align}
%\mf{Here we talk that we do not express acc in master frame through acc in IMU frame to avoid ungiven angular acc}
where
%\mf{$\lf{I_i}\vect{p}\rf{M} = -\lf{M}\vect{p}\rf{I_i}$ ?}
\begin{align}\label{eq_acc_some}
    \lf{M}\vect{a} = \lfR{M}\rf{I_i}(\lf{I_i}\vect{a} + \lf{I_i}\vect{a}_{inertial}).
\end{align}
\begin{align}
    \lf{I_i}\vect{a}_{inertial} = ([\lf{I_i}\vect{\omega}]_\times^2 + [\lf{I_i}\vect{\dot \omega}]_\times)\lf{I_i}\vect{p}\rf{M}.
\end{align}
or
\begin{align}%\label{eq_}
    %([\lf{I_i}\vect{\omega}]_\times^2 + [\lf{I_i}\vect{\dot \omega}]_\times)\lf{I_i}\vect{p}\rf{M} 
    \lf{I_i}\vect{a}_{inertial} 
    = \lfR{I_i}\rf{M} ([\lf{M}\vect{\omega}]_\times^2 + [\lf{M}\vect{\dot \omega}]_\times) \lfR{M}\rf{I_i} \lf{I_i}\vect{p}\rf{M}
\end{align}

\subsection{Averaged Virtual Estimator}\label{sub_baseline_acc}

Given multiple gyroscope sensor readings, one can estimate overall orientation by fusing all available data into a virtual angular velocity:
\begin{align}
    \lf{V}\hat{\vect{a}} = \frac{1}{N}\sum_{i=1}^N \lfR{V}\rf{I_i} (\lf{I_i}\tilde{\vect{a}} - \hat{\vect{b}}_{a_i}) + \lf{I_i}\vect{a}_{inertial}
    %([\lf{I_i}\vect{\omega}]_\times^2 + [\lf{I_i}\vect{\dot \omega}]_\times)\lf{I_i}\vect{p}\rf{V},
    \label{eq_baseline_acc}
\end{align}
where $N$ is the number of IMUs and $\lfR{V}\rf{I_i}$ is the rotation to transform IMU measurements to the virtual frame $\{V\}$ under assumption of independent noise processes with the same parameters in~(\ref{eq_perf_gyro_cont})~and~(\ref{eq_ct_byas}), matrix $C$ is not shown.

\color{black}

==> archive/_04b_acc_begin_method.tex <==
\cg

\section*{\mf{BAC ACC} }\label{sec_approach_acc}

\subsection{Stationary IMU Parameters Estimation}\label{sec_static_optim_acc}

States and parameters to be estimated are $\mf{\lf{W}\vect{v}^{i}\rf{M}(t_k)), \vect{g}?}$
\begin{align}
    \Theta_i = \{\lf{W}\vect{p}^{i}\rf{M}(t_k)), \vect{b}_a^i(t_k), C_{i_a}, \Ln(\, \lfR{I_g}^i\rf{I_a}\,)\}.
\end{align}
The number of the variables is $(6K + 12)N$ for $N$ IMU sensors and $K$ timestamps.

Assuming eqs.~(\ref{eq_cor_gyro_dis}),~(\ref{eq_bias_dis}),~(\ref{eq_mrots_dis}),~(\ref{eq_omega_rot}), the cost function given the values is the following for each IMU
\begin{align*}
    \mathcal{L}_i(\Theta_i) =& \sum_{k=0}^K \left\| \lf{W}\vect{p}^{\scriptscriptstyle GT}\rf{M}(t_k) - \lf{W}\vect{p}^{i}\rf{M}(t_k) \right\|_{\Sigma_{p}}^2\\
    +& \sum_{k=0}^K \left\| \lf{W}\vect{v}^{\scriptscriptstyle GT}\rf{M}(t_k) - \lf{W}\vect{v}^{i}\rf{M}(t_k) \right\|_{\Sigma_{v}}^2\mf{?}\\
    +& \sum_{k=0}^{K-1} \left\| \Delta \vect{b}_a^i(t_k) + \gamma \vect{b}_a^i(t_k)\right\|_{\Sigma_{\vect{n}_{b_a}}}^2, \numberthis
    \label{eq_loss_acc}
\end{align*}
where the first term is the error in orientation and the second term is condition to bias, $\lfR{M}^{\scriptscriptstyle GT}\rf{W}(t_k)$ is ground truth data provided by Master sensor, $\lfR{W}^i\rf{M}(t_k)$ is orientation estimate, %$\lf{I_i}\vect{\omega}$
$\Sigma_p$ is a covariance matrix described in~\cite{forster2015supplementary}~and~\cite{sola2018micro}.

The final cost of all IMU measurements to be minimized is
\begin{align}
    \mathcal{L}(\Theta) =& \sum_{i=0}^N \mathcal{L}_i(\Theta_i) \to \min_{\Theta}.
    \label{eq_final_loss_acc}
\end{align}

\subsection{Time-dependent IMU Parameters Estimation}

$\Theta_i~=~ \{\lf{W}\vect{p}^{i}\rf{M}(t_k), \vect{b}_a^i(t_k)\}$, $6KN$ values in total + \mf{+v}.  

\cb

==> archive/_04c_acc_end_method.tex <==
\cg\subsubsection{BAC-accelerometer}\label{sec_bac_acc}

\mf{rewrite}
%\begin{equation}
%\begin{aligned}
%    &\lf{W}\vect{p}\rf{M}(t_{k+1}) = \lfR{W}\rf{I}(t_k+1) \lf{I}\vect{p}\rf{M} + \lf{W}\vect{p}\rf{I}(t_{k+1})\\
%    \\
%    &=\lfR{W}\rf{I}(t_k+1) \lf{I}\vect{p}\rf{M} + \lf{W}\vect{p}\rf{I}(t_{k}) + \lf{W}\vect{v}\rf{I}(t_{k}) \Delta t_k + \frac{1}{2}\lf{I}\vect{\alpha}(t_k) \Delta t_k^2\\
%    \\
%    &= \lfR{W}\rf{I}(t_k+1) \lf{I}\vect{p}\rf{M} + \lf{W}\vect{p}\rf{I}(t_{k}) + \lf{W}\vect{v}\rf{I}(t_{k}) \Delta t_k + \frac{1}{2}( \lfR{W}\rf{I}(t_{k})\lf{I}\vect{a}(t_k) - \vect{g})\Delta t_k^2\\
%    \\
%    &= \lfR{W}\rf{I}(t_k+1) \lf{I}\vect{p}\rf{M} + \lf{W}\vect{p}\rf{I}(t_{k}) + \lf{W}\vect{v}\rf{I}(t_{k}) \Delta t_k + \frac{1}{2}( \lfR{W}\rf{I}(t_{k})\lf{I}\vect{a}(t_k) - \vect{g})\Delta t_k^2
%\end{aligned}
%\end{equation}


%\TODO{this next sencence is not clear. Also what is the second rotation with M?} 
Below is the description of the BAC approach.

There are $p$ last reference $\lfR{W}^{\scriptscriptstyle GT}\rf{M}(t_k)$ and estimated $\lfR{W}^M\rf{M}(t_k)$ orientations of the Master of the second stage. %for $k \in [K-p, K]$. 
%for every IMU $i \in [1,N]$. 
%$\lfR{W}^{\scriptscriptstyle GT}\rf{M}(t_k) \lfR{M}\rf{I_i}$ and $\lfR{W}^i\rf{M}(t_k) \lfR{M}\rf{I_i}$ respectively.\\
The orientation error for IMU $i$ and timestamp $k$ expressed in the respective IMU frame~$i$ is 
\begin{align*}
    \vect{e}_{i}(t_k) &= %\lf{W}\vect{p}^{\scriptscriptstyle GT}\rf{M}(t_k) - \lf{W}\vect{p}^{i}\rf{M}(t_k)\\
    \lf{W}\vect{p}^{\scriptscriptstyle GT}\rf{I}(t_k) - \lf{W}\vect{p}^{i}\rf{I}(t_k)\text{\mf{revisit index i placement}}\\
    &= (\lf{W}\vect{p}^{\scriptscriptstyle GT}\rf{M}(t_k) - \lfR{W}^{\scriptscriptstyle GT}\rf{M}(t_k) \lfR{M}\rf{I_i})\\
    &- (\lf{W}\vect{p}^{i}\rf{M}(t_k) - \lfR{W}\rf{M}(t_k) \lfR{M}\rf{I_i})
    %&= \Ln\left( \lfR{I_i}\rf{M} \lfR{M}^{\scriptscriptstyle GT}\rf{W}(t_k) \lfR{W}^i\rf{M}(t_k) \lfR{M}\rf{I_i} \right). \numberthis
\end{align*}

This is used: $\lfp{W}\rf{M} = \lfR{W}\rf{I} \lfp{I}\rf{M} + \lfp{W}\rf{I}$


Here, the mapping of the error in the Master to the IMU frames has been performed.
The mapping allows the algorithm to capture the contribution of measurements of each single axis of IMU to three-dimensional error vector 
\begin{align}
    \vect{e}_{i} = [e^x_i, e^y_i, e^z_i]^\top.
\end{align}

Then we choose the best axis from the homonymous axes of the IMUs. This is done by MSE criterion of the sets of errors $e^\alpha_i$ in time instances $t_{K-p}$,~$t_{K-p+1}$,~\dots,~$t_{K}$ for every axis $\alpha~\in \{x,y,z\}$ ($\alpha~\in \{1,2,3\}$ is used interchangeably) with the assumption that chosen axes are not coplanar:
\begin{align}
    i_{best}^\alpha = \arg \min_i \sum_{k=K-p}^K | e^\alpha_i (t_k)|^2
    \label{eq_vot_tule_acc}
\end{align}

We do it three times for every axis to compose axes of the virtual IMU. Thus, on this step the set of three non-coplanar axes \begin{align}
    \{i_{best}^x, i_{best}^y, i_{best}^z\}
    \label{eq_best_axes_acc}
\end{align}
from the set of IMU sensors for open-loop estimation have been chosen by criterion (\ref{eq_vot_tule}). 
%We call \ma{estimates} of scalar angular velocities of these axes by $\omega_{i_{best}}^x$, $\omega_{i_{best}}^y$, $\omega_{i_{best}}^z$ respectively.

The next step is the final composition of the axes and their measurements to assemble accurate distributed single virtual IMU measurements. We match axes of the virtual IMU with the Master frame for simplicity, but there are no limitations on the position and orientation of the virtual IMU. 
%For this consider now a problem of expression of non-coplanar elements of angular velocities of arbitrary chosen IMUs via angular velocity in the Master frame:
For this, consider now a problem of expression of angular velocity in the Master frame via non-coplanar elements of angular velocities 
$\lf{I_i}\omega^x,~\lf{I_j}\omega^y$ and $\lf{I_k}\omega^z$ 
of arbitrary chosen IMUs~$i$,~$j$~and~$k$:
\begin{align}\label{eq_map_acc}
    \lf{M}\vect{a} = B \cdot \begin{bmatrix} \lf{I_i}a^x + \lf{I_i} a_{inertial}^x\\ \lf{I_j}a^y + \lf{I_j} a_{inertial}^y\\ \lf{I_k}a^z + \lf{I_k} a_{inertial}^z \end{bmatrix},
\end{align}

where $A \in \mathbb{R}^{3\times3}$ is a linear mapping that is needed to be found. The matrix $A$ is non-orthonormal and does not belong to $SO(3)$ because the homonymous axes of different IMUs do not have to be coplanar in general. The inverse of $A$ can be obtained by exploring element by element of the  vector
\begin{align}%\label{eq_}
    %\lf{I_i}\vect{a} &= \lfR{I_i}\rf{M}\lf{M}\vect{a} - ([\lf{I_i}\vect{\omega}]_\times^2 + [\lf{I_i}\vect{\dot \omega}]_\times)\lf{I_i}\vect{p}\rf{M}\\
    %&= \lfR{I_i}\rf{M}\lf{M}\vect{a} - \lfR{I_i}\rf{M} ([\lf{M}\vect{\omega}]_\times^2 + [\lf{M}\vect{\dot \omega}]_\times) \lfR{M}\rf{I_i} \lf{I_i}\vect{p}\rf{M}
    \lf{I_i}\vect{a} &= \lfR{I_i}\rf{M}\lf{M}\vect{a} - \lf{I_i}\vect{a}_{inertial}
\end{align}
which is the inverse relation in (\ref{eq_omega_rot}). This gives each component of the angular velocity as a dot product of
\begin{align}\label{eq_comp_acc}
    \lf{I_i} a^\alpha = \lf{I_i} \vect{r}^\alpha \rf{M} \lf{M}\vect{a} - \lf{I_i} a_{inertial}^\alpha,
\end{align}
for every axis $\alpha$ of $\lf{I_i}\vect{a}$, where the row vector $\vect{r}^\alpha \rf{M}$ is the $\alpha$-th row of $\lfR{I_i}\rf{M}$. 
%\begin{align}
%    \lf{I_i} a_{inertial}^\alpha = (\lfR{I_i}\rf{M}([\lf{M}\vect{\omega}]_\times^2 + [\lf{M}\vect{\dot \omega}]_\times) \lfR{M}\rf{I_i} \lf{I_i}\vect{p}\rf{M})^\alpha
%\end{align}

%Using rule~(\ref{eq_comp}) one can concatenate~(\ref{eq_omegas}) and get
By stacking all the velocity components we obtain
\begin{equation}
    \begin{aligned}
        \begin{bmatrix} \lf{I_i}a^x\\ \lf{I_j}a^y\\ \lf{I_k}a^z \end{bmatrix} = 
        \begin{bmatrix}
            \lf{I_i} \vect{r}^x \rf{M}\\
            \lf{I_j} \vect{r}^y \rf{M}\\
            \lf{I_k} \vect{r}^z \rf{M}
        \end{bmatrix} \lf{M}\vect{a} - 
        \begin{bmatrix} 
            \lf{I_i} a_{inertial}^x\\
            \lf{I_j} a_{inertial}^y\\
            \lf{I_k} a_{inertial}^z
        \end{bmatrix}.
    \end{aligned}
\end{equation}

and finally,
\begin{equation}
    \begin{aligned}
        \lf{M}\vect{a} = 
        \begin{bmatrix}
            \lf{I_i} \vect{r}^x \rf{M}\\
            \lf{I_j} \vect{r}^y \rf{M}\\
            \lf{I_k} \vect{r}^z \rf{M}
        \end{bmatrix}^{-1}
        \begin{bmatrix} 
            \lf{I_i}a^x + \lf{I_i} a_{inertial}^x\\
            \lf{I_j}a^y + \lf{I_j} a_{inertial}^y\\
            \lf{I_k}a^z  +\lf{I_k} a_{inertial}^z
        \end{bmatrix}.
    \end{aligned}
\end{equation}
%\begin{equation}
%    \begin{aligned}
%        \lf{M}\vect{a} = 
%        \begin{bmatrix}
%            \lf{I_i} \vect{r}^x \rf{M}\\
%            \lf{I_j} \vect{r}^y \rf{M}\\
%            \lf{I_k} \vect{r}^z \rf{M}
%        \end{bmatrix}^{-1} \left(\rule{0cm}{0.9cm} \begin{bmatrix} \lf{I_i}a^x\\ \lf{I_j}a^y\\ \lf{I_k}a^z \end{bmatrix} + 
%        \begin{bmatrix} 
%            \lf{I_i} a_{inertial}^x\\
%            \lf{I_j} a_{inertial}^y\\
%            \lf{I_k} a_{inertial}^z
%        \end{bmatrix} \right).
%    \end{aligned}
%\end{equation}


is the solution of~(\ref{eq_map_acc}).

%Angular velocities of rigidly connected IMUs measured in common frame are equal. Thus, we can drop (\ref{eq_omega_rot}) leads to $\lf{M}\vect{\omega}_i = \lf{M}\vect{\omega}_j = \lf{M}\vect{\omega}$, where $\lf{M}\vect{\omega}$ is the reference \GF{remove pair j and only refer i and the refence}:
%\begin{align}
%    \lf{M}\vect{\omega} = \lfR{M}\rf{I_i} \lf{I_i}\vect{\omega}.
%\end{align}

%For this we express 
%The inverse of the rotation gives angular velocity $\lf{I_i}\vect{\omega}$ via $\lf{M}\vect{\omega}$:
%\GF{one can invert this expression and obtain:}
%\begin{align}
%    \lf{I_i}\vect{\omega} = \lfR{I_i} \rf{M} \lf{M}\vect{\omega}
%\end{align}
%and for every axis $\alpha$ of $i$-th IMU:
%\begin{align}
%    \lf{I_i}\omega^\alpha = \lf{I_i} R^\alpha \rf{M} \lf{M}\vect{\omega},
%\end{align}
%where $\lf{I_i} R^\alpha \rf{M}$ is an $\alpha$-th row of matrix $\lfR{I_i}\rf{M}$.\GF{remove innecessary equations, explain the process of selecting axis as in (17) and write crelarly when it becomes NON-Orthonormal R}

%Concatenation of three arbitrary chosen pair $\alpha$ -- IMU, namely \ma{$\{x, I_i\}$, $\{y, I_j\}$, $\{z, I_k\}$}, constitutes the system of linear equations in matrix form:
%\ma{\begin{align}
%    \begin{bmatrix} \lf{I_i}\omega^x\\ \lf{I_j}\omega^y\\ \lf{I_k}\omega^z \end{bmatrix} = \begin{bmatrix} \lf{I_i} R^x \rf{M}\\ \lf{I_j} R^y \rf{M}\\ \lf{I_k} R^z \rf{M} \end{bmatrix} \lf{M}\vect{\omega}.
%\end{align}}

%Solving the system determines the angular velocities to be used for orientation estimation
%\ma{\begin{align}
%    \lf{M}\vect{\omega} = \begin{bmatrix} \lf{I_i} R^x \rf{M}\\ \lf{I_j} R^y \rf{M}\\ \lf{I_k} R^z \rf{M} \end{bmatrix}^{-1} \begin{bmatrix} \lf{I_i}\omega^x\\ \lf{I_j}\omega^y\\ \lf{I_k}\omega^z \end{bmatrix}
%    \label{eq_distr}
%\end{align}}
%if the matrix \ma{$\begin{bmatrix} \lf{I_i} R^x \rf{M}\\ \lf{I_j} R^y \rf{M}\\ \lf{I_k} R^z \rf{M} \end{bmatrix}$} 
%is invertible. \ma{For that any pair of the rows of this matrix must not be equal. It is always true if any pair of differently named axes of a pair of different IMUs does not coincide. This is the only one limitation on poses of IMUs in our method.} Here we consciously use inverse but not transpose of this matrix because orientations of \ma{IMU frames do not coincide} and thus, the matrix does not belong to $SO(3)$.

Changing superscripts $I_i$, $I_j$, $I_k$ in~(\ref{eq_distr}) on $I_{i_{best}^x}, I_{i_{best}^y}, I_{i_{best}^z}$
%those in (\ref{eq_best_axes}) 
accordingly we get BAC. As a result for the third stage, we have prepared accurate distributed IMU (\ref{eq_distr}) for open-loop orientation estimation. 

\subsection{Open-loop}
The third stage of the approach is open-loop orientation estimation by only IMUs measurements without Master aid. This is an integration of distributed IMU measurements (\ref{eq_distr}) with constant bias equal to the last estimated value in the second stage of the approach $\vect{b} = \vect{b}(t_K)$. 

As was mentioned in the Section~\ref{sec_intro}, highly dynamic motion of aerial robots or augmented and virtual reality systems require as low as possible processing time of data along with frequent updates of current state (high data rate). Using only visual data requires several tens or hundreds of milliseconds delay between events and their estimation. In these circumstances IMU sensors provide a much faster alternative and BAC outperforms state-of-the-art IMU solutions in accuracy over short time horizons. % of time without any additional aid in open-loop.

\cb

==> archive/_backup.tex <==
\section{Rigid Body Transformation IMU}\label{sec_rbt}


We will follow a different derivation for the equations. The difference is that instaead oif integrating sensor reading, we will calculate the derivative of poses (trajectory).
By following this derivation we will obtain the same result as explained on the background section with an additional term.


Poses are expressed as rigid body transformations $T \in SE(3)$.

\begin{equation}
\lfT{W}\rf{I}(t) = \begin{bmatrix} \lfR{W}\rf{I}(t) & \lf{W}p\rf{I}(t) \\ 
                              0 & 1 \end{bmatrix}
\label{eq_first}
\end{equation}


In order to differentiate a transformation $T \in \SE3$, we need to follow the chian rule and obtain 

\WORRIES{Should we use this chain rule? Is it better to use just well known $T^{-1} \dot T = [v, \omega]$?}

\TODO{check this, but then you can differentiate the translation components t}
\WORRIES{$V^{-1}$}
\begin{gather}
\lf{W}\dot{T}\rf{I}(t) = \frac{\partial T}{\partial \xi} \frac{\partial \xi}{\partial t} 
=\frac{\partial [R\Exp(\int_{0}^{dt}\omega(t')dt') p(t)]}{\partial \xi(i)} \\
= \begin{bmatrix} \lfR{W}\rf{I}(t)\cdot \omega(t)^{\land}  & V^{-1}\lf{W}\dot{p}\rf{I}(t) \\ 
                              0 & 1 \end{bmatrix} 
\end{gather}

\begin{equation}
\lf{W}\ddot{T}\rf{I}(t) = \begin{bmatrix} \lfR{W}\rf{I}(t) (\omega(t)^{\land})^2 + 
                        \lfR{W}\rf{I}(t) \dot{\omega}(t)^{\land} &
                        \lf{W}p\rf{I} \\ 
                              0 & 1 \end{bmatrix}
\label{eq_first}
\end{equation}

Expansion from the body frame
\begin{equation}
\dot{T} = T \cdot \lf{B}W
\label{eq_SE3_body}
\end{equation}


\begin{equation}
\frac{\partial \dot{T}}{\partial t} = \dot{T}W + T\dot{W} =
 T \cdot \lf{B}W^2 + T\cdot \lf{B}\dot{W}
\label{eq_SE3_diff}
\end{equation}

\begin{equation}
\lf{B}{W} = \begin{bmatrix} \lf{B}\omega(t)^{\land}) & \lf{B}v \\ 
                              0 & 0 \end{bmatrix}
\end{equation}

\begin{equation}
\lf{B}\dot{W} = \begin{bmatrix} 0 & \lf{B}a \\ 
                              0 & 0 \end{bmatrix}
\end{equation}

Piece-wise constant angular velocity and piece-wise constant acceleration.

An then integrate from the body twist $\lf{B}W$.


==============\\
Below is related kinematics for rigidly connected points A and B by transformation matrix $\lfT{B}\rf{A}$ that expresses frame A wrt. frame B. $\lf{A}x$ means $x$ in frame A. The same holds for B.

Poses of frames A and B in world frame (W) and their derivatives are connected by the following equations.
\\

\textbf{Zeroth derivative}
\begin{align*}
&& \lfT{W}\rf{A} &= \lfT{W}\rf{B} \lfT{B}\rf{A}\\
\\
\text{Expansion}
&& \lfR{W}\rf{A} &= \lfR{W}\rf{B} \lfR{B}\rf{A}\\
&& \lfp{W}\rf{A} &= \lfR{W}\rf{B} \lfp{B}\rf{A} + \lfp{W}\rf{B}
\end{align*}

\textbf{First derivative}

\begin{align*}
&& \lfdotT{W}\rf{A} &= \lfdotT{W}\rf{B} \lfT{B}\rf{A}\\
\\
\text{Expansion} && \lfR{W}\rf{A} [\lf{A}\omega]_\times &= \lfR{W}\rf{B} [\lf{B}\omega]_\times \lfR{B}\rf{A}\\
&& \lfR{W}\rf{A} \lf{A}v &= \lfR{W}\rf{B} ([\lf{B}\omega]_\times \lfp{B}\rf{A} + \lf{B}v)\\
\\
\text{Note 1} && [\lf{A}\omega]_\times &= \lfR{A}\rf{B} [\lf{B}\omega]_\times \lfR{B}\rf{A}\\
\text{or} && \lf{A}\omega &= \lfR{A}\rf{B} \lf{B}\omega\\
\text{Note 1} && \lf{A}v &= \lfR{A}\rf{B} ([\lf{B}\omega]_\times \lfp{B}\rf{A} + \lf{B}v)
\end{align*}

\textbf{Second derivative}
\begin{align*}
&& \lfddotT{W}\rf{A} &= \lfddotT{W}\rf{B} \lfT{B}\rf{A}\\
\\
\text{Ex}
&& \lfR{W}\rf{A} ([\lf{A}\omega]_\times^2 + [\lf{A}\dot{\omega}]_\times) &= \lfR{W}\rf{B} ([\lf{B}\omega]_\times^2 + [\lf{B}\dot{\omega}]_\times) \lfR{B}\rf{A}\\
%& & \lfR{W}\rf{A} ([\lf{A}\omega]_\times \lf{A}v + \lf{A}a) &= \lfR{W}\rf{B} \{([\lf{B}\omega]_\times^2 + [\lf{B}\dot{\omega}]_\times) \lfp{B}\rf{A} + [\lf{B}{\omega}]_\times \lf{B}v + \lf{B}a\}\\
&& \lfR{W}\rf{A} \lf{A}a &= \lfR{W}\rf{B} \{([\lf{B}\omega]_\times^2 + [\lf{B}\dot{\omega}]_\times) \lfp{B}\rf{A} + \lf{B}a\}\\
\\
\text{Note 1}
&& [\lf{A}\omega]_\times^2 + [\lf{A}\dot{\omega}]_\times &= \lfR{A}\rf{B} ([\lf{B}\omega]_\times^2 + [\lf{B}\dot{\omega}]_\times) \lfR{B}\rf{A}\\
\text{or} && \lf{A}\dot\omega &= \lfR{A}\rf{B} \lf{B}\dot\omega\\
\text{Note 2} && \lf{A}a &= \lfR{A}\rf{B} \{([\lf{B}\omega]_\times^2 + [\lf{B}\dot{\omega}]_\times) \lfp{B}\rf{A} + \lf{B}a\}\\
\end{align*}

$\omega, \dot \omega, v, \dot v$ IN WORLD FRAME\\

Zeroth derivative
\begin{align*}
\lfT{W}\rf{A} &= \lfT{W}\rf{B} \lfT{B}\rf{A} & \lfR{W}\rf{A} &= \lfR{W}\rf{B} \lfR{B}\rf{A}\\
& & \lfp{W}\rf{A} &= \lfR{W}\rf{B} \lfp{B}\rf{A} + \lfp{W}\rf{B}
\end{align*}

First derivative
\begin{align*}
\lfdotT{W}\rf{A} &= \lfdotT{W}\rf{B} \lfT{B}\rf{A} & [\lf{A}\omega]_\times \lfR{W}\rf{A} &= [\lf{B}\omega]_\times \lfR{W}\rf{B} \lfR{B}\rf{A}\\
& & [\lf{A}\omega]_\times \lfp{W}\rf{A} + \lf{A}v &= [\lf{B}\omega]_\times (\lfR{W}\rf{B} \lfp{B}\rf{A} + \lfp{W}\rf{B}) + \lf{B}v\\
\\
\text{Note} & & \lf{A}\omega &= \lf{B}\omega\\
\text{Note} & & \lf{A}v &= [\lf{B}\omega]_\times (\lfR{W}\rf{B} \lfp{B}\rf{A} + \lfp{W}\rf{B} - \lfp{W}\rf{A}) + \lf{B}v\\
\text{or} & & \lf{A}v &= \lf{B}v\\
\end{align*}

Second derivative
\begin{align*}
\lfddotT{W}\rf{A} &= \lfddotT{W}\rf{B} \lfT{B}\rf{A} & ([\lf{A}\omega]_\times^2 + [\lf{A}\dot{\omega}]_\times) \lfR{W}\rf{A} &= ([\lf{B}\omega]_\times^2 + [\lf{B}\dot{\omega}]_\times) \lfR{W}\rf{B} \lfR{B}\rf{A}\\
& & ([\lf{A}\omega]_\times^2 + [\lf{A}\dot{\omega}]_\times)\lfp{W}\rf{A} + [\lf{A}\omega]_\times \lf{A}v + \lf{A}a &= ([\lf{B}\omega]_\times^2 + [\lf{B}\dot{\omega}]_\times) (\lfR{W}\rf{B} \lfp{B}\rf{A} + \lfp{W}\rf{B}) + [\lf{B}{\omega}]_\times \lf{B}v + \lf{B}a\\
\\
\text{Note} & & [\lf{A}\omega]_\times^2 + [\lf{A}\dot{\omega}]_\times &= [\lf{B}\omega]_\times^2 + [\lf{B}\dot{\omega}]_\times\\
\text{or} & & \lf{A}\dot\omega &= \lf{B}\dot\omega\\
\text{Note} & & \lf{A}a &= \lf{B}a\\
\end{align*}
==============

But what is $\lfR{W}\rf{M}(t)$

\begin{equation}
\lf{M}\omega = \lfR{M}\rf{I}\lf{I}\omega
\label{eq_qq}
\end{equation}

For any rot m and omega belonging to SO3/so3

\begin{align}
\Exp (R \theta) = R \Exp (\theta) R^\top
\label{eq_qq}
\end{align}


\begin{equation}
\lfR{W}\rf{M}(t+\Delta t) = \lfR{W}\rf{M}(t) \Exp (\lf{M}\omega(t) \Delta t)
\label{eq_qq}
\end{equation}

\begin{equation}
\lfR{W}\rf{M}(t+\Delta t) = \lfR{W}\rf{M}(t) \lfR{M}\rf{I} \Exp (\lf{I}\omega(t) \Delta t) \lfR{I}\rf{M}
\label{eq_qq}    
\end{equation}

\begin{equation}
\lf{W}\theta\rf{M}(t) = \Log (\lfR{W}\rf{M}(t))
\label{eq_qq}    
\end{equation}

\begin{equation}
\lf{M}\theta\rf{I} = \Log (\lfR{M}\rf{I})
\label{eq_qq}    
\end{equation}

parameters to estimate on the first stage

$\lf{W}\theta\rf{M}(0), \lf{M}\theta\rf{I}, b(t), M, A$

TOTHINK: $\lf{W}\theta\rf{M}(0)$ can be chosen right from master data

Freezing all the parameters on the second stage

$\lf{W}\theta\rf{M}(0'), \lf{M}\theta\rf{I}, b(t) = b(0'), M, A$

Functional to be minimized is the following

\begin{equation}
\mathcal{L} = \sum_{k=0}^K \left\| \Log (\lfR{W}\rf{M}(t_k) \lfR{M}\rf{W ref}(t_k)) \right\|_{\Sigma_{\theta}}^2 + \sum_{n=0}^N \left\| \Delta b_\omega(t_n) \right\|_{\Sigma_{b}}^2
\label{eq_qq}    
\end{equation}

\begin{equation}
\Delta b_\omega(t_n) = b_\omega(t_{n+1}) - b_\omega(t_n)
\label{eq_qq}    
\end{equation}

====================================

\section{Rigid Body Transformations}\label{sec_rbt}

Assume rigid-body platform where IMU-sensor is placed. IMU has its own frame I. Any frame M rigidly connected with the platform has constant displacement and orientation wrt. frame I. M stands for Master that can be any sensor namely visual camera, depth camera, lidar or any other essential point on the platform. This transformation between rigidly connected frames M and I can be expressed through transformation matrix $\lfT{I}\rf{M}$ such that pose of Master in global frame $\lfT{W}\rf{M}$ can be expressed via pose of IMU in global frame $\lfT{W}\rf{I}$ by following equation. 


\textbf{Zeroth derivative}
\begin{align*}
&& \lfT{W}\rf{M} &= \lfT{W}\rf{I} \lfT{I}\rf{M}\\
\\
\text{Expansion}
&& \lfR{W}\rf{M} &= \lfR{W}\rf{I} \lfR{I}\rf{M}\\
&& \lfp{W}\rf{M} &= \lfR{W}\rf{I} \lfp{I}\rf{M} + \lfp{W}\rf{I}
\end{align*}

Moreover the first and second derivatives of this connection give the following results.

\textbf{First derivative}

\begin{align*}
&& \lfdotT{W}\rf{M} &= \lfdotT{W}\rf{I} \lfT{I}\rf{M}\\
\\
\text{Expansion} && \lfR{W}\rf{M} [\lf{M}\omega]_\times &= \lfR{W}\rf{I} [\lf{I}\omega]_\times \lfR{I}\rf{M}\\
&& \lfR{W}\rf{M} \lf{M}v &= \lfR{W}\rf{I} ([\lf{I}\omega]_\times \lfp{I}\rf{M} + \lf{I}v)\\
\\
\text{Note 1} && [\lf{M}\omega]_\times &= \lfR{M}\rf{I} [\lf{I}\omega]_\times \lfR{I}\rf{M}\\
\text{or} && \lf{M}\omega &= \lfR{M}\rf{I} \lf{I}\omega\\
\text{Note 2} && \lf{M}v &= \lfR{M}\rf{I} ([\lf{I}\omega]_\times \lfp{I}\rf{M} + \lf{I}v)
\end{align*}

\textbf{Second derivative}
\begin{align*}
&& \lfddotT{W}\rf{M} &= \lfddotT{W}\rf{I} \lfT{I}\rf{M}\\
\\
\text{Ex}
&& \lfR{W}\rf{M} ([\lf{M}\omega]_\times^2 + [\lf{M}\dot{\omega}]_\times) &= \lfR{W}\rf{I} ([\lf{I}\omega]_\times^2 + [\lf{I}\dot{\omega}]_\times) \lfR{I}\rf{M}\\
%& & \lfR{W}\rf{M} ([\lf{M}\omega]_\times \lf{M}v + \lf{M}a) &= \lfR{W}\rf{I} \{([\lf{I}\omega]_\times^2 + [\lf{I}\dot{\omega}]_\times) \lfp{I}\rf{M} + [\lf{I}{\omega}]_\times \lf{I}v + \lf{I}a\}\\
&& \lfR{W}\rf{M} \lf{M}a &= \lfR{W}\rf{I} \{([\lf{I}\omega]_\times^2 + [\lf{I}\dot{\omega}]_\times) \lfp{I}\rf{M} + \lf{I}a\}\\
\\
\text{Note 1}
&& [\lf{M}\omega]_\times^2 + [\lf{M}\dot{\omega}]_\times &= \lfR{M}\rf{I} ([\lf{I}\omega]_\times^2 + [\lf{I}\dot{\omega}]_\times) \lfR{I}\rf{M}\\
\text{or} && \lf{M}\dot\omega &= \lfR{M}\rf{I} \lf{I}\dot\omega\\
\text{Note 2} && \lf{M}a &= \lfR{M}\rf{I} \{([\lf{I}\omega]_\times^2 + [\lf{I}\dot{\omega}]_\times) \lfp{I}\rf{M} + \lf{I}a\}\\
\end{align*}

But what is $\lfR{W}\rf{M}(t)$

\begin{equation}
\lf{M}\omega = \lfR{M}\rf{I}\lf{I}\omega
\label{eq_qq}
\end{equation}

=======================
\section{State variables and Frames}\label{sec_frames}

% 
The input variables are the readings from the IMU sensor, i.e., acceleration $a$ and angular velocity $\omega$ each of them measuring their corresponding variables in three axis.
The state variables are position $p \in \mathbb{R}^3$, orientation $\theta \in SO(3)$, velocity $v \in \mathbb{R}^3$ and the corresponding bias to the accelerometer $b_a$ and bias for the gyroscope $b_{\omega}$ 
=========================

\section{MIMU auction}

Suppose we want to utilize measurements from different imus represented in Master frame.

equations



For any rot m and omega belonging to SO3/so3

\begin{align}
\Exp (R \theta) = R \Exp (\theta) R^\top
\label{eq_qq}
\end{align}


\begin{equation}
\lfR{W}\rf{M}(t+\Delta t) = \lfR{W}\rf{M}(t) \Exp (\lf{M}\omega(t) \Delta t)
\label{eq_qq}
\end{equation}

\begin{equation}
\lfR{W}\rf{M}(t+\Delta t) = \lfR{W}\rf{M}(t) \lfR{M}\rf{I} \Exp (\lf{I}\omega(t) \Delta t) \lfR{I}\rf{M}
\label{eq_qq}    
\end{equation}

\begin{equation}
\lf{W}\theta\rf{M}(t) = \Ln (\lfR{W}\rf{M}(t))
\label{eq_qq}    
\end{equation}

\begin{equation}
\lf{M}\theta\rf{I} = \Ln (\lfR{M}\rf{I})
\label{eq_qq}    
\end{equation}

parameters to estimate on the first stage

$\lf{W}\theta\rf{M}(0), \lf{M}\theta\rf{I}, b(t), M, A$

TOTHINK: $\lf{W}\theta\rf{M}(0)$ can be chosen right from master data

Freezing all the parameters on the second stage

$\lf{W}\theta\rf{M}(0'), \lf{M}\theta\rf{I}, b(t) = b(0'), M, A$

Functional to be minimized is the following

\begin{equation}
\mathcal{L} = \sum_{k=0}^K \left\| \Ln (\lfR{W}\rf{M}(t_k) \lfR{M}\rf{W ref}(t_k)) \right\|_{\Sigma_{\theta}}^2 + \sum_{n=0}^N \left\| \Delta b_\omega(t_n) \right\|_{\Sigma_{b}}^2
\label{eq_qq}    
\end{equation}

\begin{equation}
\Delta b_\omega(t_n) = b_\omega(t_{n+1}) - b_\omega(t_n)
\label{eq_qq}    
\end{equation}


where $t_k$ timestamp of every IMU sample, $t_n$ is timestamp (HOWTO explain)

We model biases as piece-wise constant ones in relatively long horizon. Bias is constant within 30-samples period.

number of parameters for single IMU system

1 Sample: 3+3+6+3+9 = 24

h samples (constant bias horizon): (3+3)*h+6+3+9 = 

h*l samples: 3(2h+1)l + 15


% Cost function

Batch optimization of this factors. \TODO{}

=================================
Briefly:\\
\cite{olson2011apriltag} - AprilTag CITED\\
\cite{titterton2004strapdown} - common gyro and acc model. strapdown CITED\\
\cite{forster2015imu} - preintegration on manifold CITED\\
\cite{furgale2013} - Unified Temporal and Spatial Calibration for Multi-Sensor Systems\\
\cite{kevin2017modern} - RB-kinematics, book CITED\\
\cite{wuest2019online} and \cite{svacha2018inertial} and \cite{svacha2019inertial} - VN/VIN + drag forces model\\
\cite{nikolic2016characterisation} (\cite{nikolic2015maximum}) - Noise model / extrinsic and intrinsic parameters / device / application (thesis by Nikolic)\\
\cite{sola2018micro} - A micro Lie Theory\\
\cite{furgale2012continuous} - continuous time optimisation by splines. Before Kalibr CITED\\
\cite{moakher2002means} - means and averaging in groups of rotations\\
\cite{huang2019visual} - Visual-inertial navigation: A concise review. Tightly-Loosely coupled and other info\\
\cite{nilsson2016inertial} and \cite{skog2016inertial} - MIMU! Inertial sensor arrays. Review with equation or filters frameworks. Higher accuracy Higher reliability and uncertainties estimation Higher dynamic measurement range Estimation of angular motion from accelerometer data Direct estimation of angular acceleration\\
\cite{skog2014open} - MIMU! platform. To detect and isolate sensor failures, thereby
increasing the reliability and integrity of the sensor system.\\
\cite{skog2006calibration} - calibration of MEMS IMU\\
TORECALL \cite{d2018calibration1} and \cite{d2018calibration2} calibration of MEMS IMU\\
\cite{solin2018inertial} - inertial odometry using iphone and zero-velocity updates and
pseudo-measurements limiting the momentary speed algorithm\\
\cite{rehder2017camera} - camera/imu calibration revisited. Kalibr, the same hw sensor\\
\cite{rhudy2012fusion} - two fusion methods of GPS and Redundant IMU Data\\
\cite{eckenhoff2019multi} - Multi-Camera Visual-Inertial Navigation with Online Intrinsic and Extrinsic Calibration cam intr and both extr\\
TOREAD \cite{kim2017line} - On-Line Initialization and Extrinsic Calibration of an Inertial Navigation System With a Relative Preintegration Method on Manifold\\
\cite{eckenhoff2019sensor} - MIMU! Sensor-Failure-Resilient Multi-IMU Visual-Inertial Navigation\\
\cite{leutenegger2015keyframe} - Keyframe-Based Visual-Inertial Odometry UsingNonlinear Optimization to mention optimization instead of *KF methods\\
\cite{zhang2019lightweight} - MIMU! trials to improve accuracy by averaging MIMU measurements\\
\cite{crassidis2006sigma} - discrete model of bias explanation\\
\cite{rehder2016extending} - Kalibr\\
\cite{wang2019optimized} - Optimized Multi-Position Calibration Method with Nonlinear Scale Factor for Inertial Measurement Units\\
\cite{barfoot2017} - State Estimation for Robotics, Barfoot book\\


\cite{nilsson2016inertial} and \\
OK\cite{skog2016inertial} - MIMU! Inertial sensor arrays. Review with equation or filters frameworks. Higher accuracy Higher reliability and uncertainties estimation Higher dynamic measurement range Estimation of angular motion from accelerometer data Direct estimation of angular acceleration\\
OK\cite{skog2014open} - MIMU! platform. To detect and isolate sensor failures, thereby
increasing the reliability and integrity of the sensor system.\\
OK\cite{eckenhoff2019sensor} - MIMU! Sensor-Failure-Resilient Multi-IMU Visual-Inertial Navigation\\
OK\cite{zhang2019lightweight} - MIMU! trials to improve accuracy by averaging MIMU measurements\\
OK\cite{rhudy2012fusion} - three fusion methods of GPS and Redundant IMU Data\\
OK\cite{wang2019optimized} - Optimized Multi-Position Calibration Method with Nonlinear Scale Factor for Inertial Measurement Units\\
TOINTRO\cite{huang2019visual} - Visual-inertial navigation: A concise review. Tightly-Loosely coupled and other info\\
NOTNEEDED \cite{d2018calibration1} and \cite{d2018calibration2} calibration of MEMS IMU\\
\cite{rehder2016extending} - Kalibr\\
===============================


==> archive/_pres.tex <==
\section{Formulas for Presentation}%\label{}

\begin{align}
    \pmb{p} (t) =& \int_0^t \int_0^t \pmb{a}(t') dt'^2\\
    \pmb{\theta}(t) =& \int_0^t \pmb{\omega}(t') dt'\\
\end{align}

\begin{align}
    \ac \neq & \; \ac_I\\
    \om \neq & \; \om_I\\
\end{align}

\begin{align}
    \ac = & \; R \, \ac_I\\
    \om = & \; R \, \om_I\\
    R = & \, \Exp(\pmb{\theta}) \in SO(3)
\end{align}

\begin{align}
    \ac_I \neq & \; \tilde \ac_I\\
    \om_I \neq & \; \tilde \om_I
\end{align}

\begin{align}
    \ac_I(t) = & \; A_a \tilde \ac_I(t) + \pmb{b}_a(t) + \pmb{\eta}_a(t)\\
    \om_I(t) = & \; A_\omega \tilde \om_I(t) + \pmb{b}_\omega(t) + \pmb{\eta}_\omega(t)
\end{align}
%b
\begin{align}
    \dot{\pmb{b}}_a(t) = & \; \pmb{\nu}_a(t)\\
    \dot{\pmb{b}}_\omega(t) = & \; \pmb{\nu}_\omega(t)
\end{align}

%\begin{align}
%    \ac_I(t_k) = & \; A_a \tilde \ac_I(t_k) + \pmb{b}_a(t_k) + \pmb{\eta}_a(t_k)\\
%    \om_I(t_k) = & \; A_\omega \tilde \om_I(t_k) + \pmb{b}_\omega(t_k) + \pmb{\eta}_\omega(t_k)
%\end{align}
%bd
%\begin{align}
%    \pmb{b}_a(t_k) = \pmb{b}_a(t_{k-1}) + \pmb{\nu}_a(t_k)\\
%    \pmb{b}_\omega(t_k) = \pmb{b}_\omega(t_{k-1}) + \pmb{\nu}_\omega(t_k)
%\end{align}

\begin{align}
    \ac_{I k} &= A_a \tilde \ac_{I k} + \pmb{b}_{a k} + \pmb{\eta}_{a k}\\
    \om_{I k} &= A_\omega \tilde \om_{I k} + \pmb{b}_{\omega k} + \pmb{\eta}_{\omega k}
\end{align}
%bd
\begin{align}
    \pmb{b}_k^a &= \pmb{b}_{k-1}^a + \pmb{\nu}_k^a\\
    \pmb{b}_k^\omega &= \pmb{b}_{k-1}^\omega + \pmb{\nu}_k^\omega
\end{align}

%\begin{align}
%    R(t_{k+1}) &= R(t_k) \Exp(\pmb{\omega}_I(t_k) \Delta t)\\
%    \pmb{v}(t_{k+1}) &= \pmb{v}(t_k) + R(t_k) \: \pmb{a}_I(t_k) \Delta t\\
%    \pmb{p}(t_{k+1}) &= \pmb{p}(t_k) + \pmb{v}(t_k)\Delta t + R(t_k) \: \pmb{a}_I(t_k) \Delta t^2/2\\
%\end{align}
\begin{align}
    R_{k+1} &= R_k \Exp(\pmb{\omega}_{I k} \Delta t)\\
    \pmb{v}_{k+1} &= \pmb{v}_k + R_k \: \pmb{a}_{I k} \Delta t\\
    \pmb{p}_{k+1} &= \pmb{p}_k + \pmb{v}_k\Delta t + R_k \: \pmb{a}_{I k} \; \Delta t^2/2\\
\end{align}
$\chi = \{
    R_k,
    \pmb{v}_k,
    \pmb{p}_k,
    \pmb{b}_k^a,
    \pmb{b}_k^\omega
    \: | \; k=1..N
\}$\\
\\

$$\chi* = \arg \min_\chi \log \mathcal{L}$$\\
\\
$\log \mathcal{L} = \sum_{k=1}^N \log \mathcal{L}_k$\\
\\
$\log \mathcal{L}_k = \|\Delta R_k\|_{\Sigma_R}^2 + \|\Delta \pmb{v}_k\|_{\Sigma_{\pmb{v}}}^2 + \|\Delta \pmb{p}_k\|_{\Sigma_{\pmb{p}}}^2 + \|\Delta \pmb{b}_k^a \|_{\Sigma_{\pmb{b}_k^a}}^2 + \|\Delta \pmb{b}_k^\omega \|_{\Sigma_{\pmb{b}_k^\omega}}^2$\\
\\
\begin{align}
    \Delta \pmb{v}_k &= \pmb{v}_k - \pmb{v}_k^{ref}\\
    \Delta \pmb{p}_k &= \pmb{p}_k - \pmb{p}_k^{ref}\\
    \Delta R_k &= R_k - R_k^{ref}\\
    \Delta \pmb{b}_k &= \pmb{b}_k-\pmb{b}_{k-1}
\end{align}
\\
$\log \mathcal{L} = \sum_{i=1}^M \sum_{k=1}^N \log \mathcal{L}_k^i + \mathcal{R}_k$\\
\\
$\mathcal{R}_k = \| \pmb{p}_k^A - \pmb{p}_k^B - \pmb{p}_k^{AB}\|_{\Sigma_{p}}^2 + \| \Ln((R_k^A)^T R_k^B R_k^{AB})\|_{\Sigma_{R}}^2 + \dots$\\
\\

Model:
$$a_I(t_k) = A_a \amk + b_a(t_k) + \eta_a(t_k),\hspace*{8pt} b_a(t_k + \Delta t) = b_a(t_k) + \nu_a(t_k)$$
$$\omega_I(t_k) = A_\omega \omk + b_\omega(t_k) + \eta_\omega(t_k),\hspace*{8pt} b_\omega(t_k) = b_\omega(t_k)  + \nu_\omega(t_k)$$\\
\\
Exponent map
skatch\\
\\
$R = \Exp(\theta)$\\
\\
\\
$v(t_0) = v_0,\hspace*{4pt} r(t_0) = r_0,\hspace*{4pt} R(t_0) = R_0$\\
\\
$R(t_{k} + \Delta t) = R(t_k) \Exp(\omega_I(t_k) \Delta t)$\\
\\
$v(t_{k} + \Delta t ) = v(t_k) + R(t_k) \: a_I(t_k) \Delta t$\\
\\
$r(t_{k} + \Delta t) = r(t_k) + v(t_k)\Delta t + R(t_k) \: a_I(t_k) \Delta t^2/2$\\
\\
%$\theta_I(t_{k+1}) = \Ln(R(t_{k+1}))$
\\
Parameters\\
\\
$\chi = \{r(t_k), v(t_k), R(t_k), b_a (t_k), b_\omega(t_k)\}$\\
\\
$$\chi* = \arg \min_\chi \log \mathcal{L}$$\\
Factors\\
\\
$\log \mathcal{L} = \sum_{k=1}^N \log \mathcal{L}_k$\\
\\
$\log \mathcal{L}_k = \|\Delta r(t_k)\|_{\Sigma_r}^2 + \|\Delta v(t_k)\|_{\Sigma_v}^2 + \|\Delta R_k\|_{\Sigma_R}^2 + \|\Delta b_a (t_k)\|_{\Sigma_{b_a}}^2 + \|\Delta b_\omega (t_k)\|_{\Sigma_{b_g}}^2$\\
\\
$\Delta r(t_k) = r(t_k) - r_{ref}(t_k)$\\
\\
$\Delta v(t_k) = v(t_k) - v_{ref}(t_k)$\\
\\
$\Delta R(t_k) = \Ln(R^T(t_k) R_{ref}(t_k))$\\
\\
$\Delta b_a (t_k) = b_a(t_k)-b_a(t_{k-1})$\\
\\
$\Delta b_\omega (t_k) = b_\omega(t_k)-b_\omega(t_{k-1})$\\
\\
RB\\
\\
$0 = r_B - (r_A + r_{AB})$\\
%\\
$I = R_B^T R_A R_{AB}$\\
%\\
$0 = v_B - (v_A + f(r_{AB}, \omega_A, \omega_B))$\\
%\\
$0 = \omega_B - h(\omega_A, R_{AB})$\\
%\\
$0 = a_B - (a_A + g(r_{AB}, v_a, v_b, \omega_A, \omega_B, R_{AB}))$\\
\\
$r_I(t), \theta_I(t)$\\
\\
$\am, \om$\\
\\
$\pmb{\omega} = \frac{d\pmb{\theta}}{dt}$\\
\\
$\pmb a = \frac{d^2 \pmb{p}}{dt^2}$\\


$\Delta \pmb{\theta} = \Ln (\Exp(\pmb{\theta}_1)^T\Exp(\pmb{\theta}_2))$\\
\\
$\Delta \pmb{\theta} = \pmb{\theta}_2 - \pmb{\theta}_1$\\
\\
$R \in SO(3)$\\
\\
$\pmb{\theta}^{\wedge} = \begin{bmatrix}
0 & -\theta_z & \theta_y\\
\theta_z & 0 & -\theta_x\\
-\theta_y & \theta_x & 0
\end{bmatrix}$\\
\\
$\Exp(\pmb{\theta})$\\
\\
$\exp(\pmb{\theta}^{\wedge})$\\
\\
$\Ln(R)$\\
\\
$\ln(R)$\\
\\
$\pmb{\theta}^{\wedge}$\\
\\
$(\pmb{\theta}^{\wedge})^{\vee}$\\
\\
$R$\\
\\
$\pmb{\theta}$\\
\\
$\pmb{\theta}^{\wedge}$\\
\\
$R \dot R = \pmb{\omega}^{\wedge}$\\
\\
$R_{k+1} = \Exp(\theta_k + \pmb{\omega}_{I k} \Delta t)$\\
\\
$\pmb{p}_A - \pmb{p}_B - R_B \pmb{p}_{AB}$\\
\\
$\Ln(R_A^T R_B R_{BA})$\\
\\
$R_A \pmb{v}_A - R_B (\oh_B \; \pmb{p_{BA}} + \pmb{v}_B)$\\
\\
$\Ln((R_A \oh_A)^T R_B \oh_B R_{BA})$\\
\\
$R_A (\oh_A\pmb{v}_A + \pmb{a}_A) - R_B (\fob \pmb{p}_{BA} + \oh_B \pmb{v}_B + \pmb{a}_B)$\\
\\
$\Ln((R_A \foa)^T R_B \fob R_{BA})$\\
\\
\begin{align*}
    \mathcal{R} &= \| \pmb{p}_A - \pmb{p}_B - R_B \pmb{p}_{AB} \|_{\Sigma_{p}}^2 &(p)\\
    &+ \| \Ln(R_A^T R_B R_{BA}) \|_{\Sigma_{\theta}}^2 &(\theta)\\
    &+ \| R_A \pmb{v}_A - R_B (\oh_B \; \pmb{p_{BA}} + \pmb{v}_B) \|_{\Sigma_{v}}^2 &(v)\\
    &+ \| \Ln((R_A \oh_A)^T R_B \oh_B R_{BA}) \|_{\Sigma_{\omega}}^2 &(\omega)\\
    &+ \| R_A (\oh_A\pmb{v}_A + \pmb{a}_A) - R_B (\fob \pmb{p}_{BA} + \oh_B \pmb{v}_B + \pmb{a}_B) \|_{\Sigma_{a}}^2  &(a)\\
    &+ \| \Ln((R_A \foa)^T R_B \fob R_{BA}) \|_{\Sigma_{\dot \omega}}^2 &(\dot \omega)
\end{align*}

